Centimeter-Wave Free-Space Time-of-Flight Imaging

Depth cameras are emerging as a cornerstone modality with diverse applications that directly or indirectly rely on measured depth, including personal devices, robotics, and self-driving vehicles. Although time-of-flight (ToF) methods have fueled these applications, the precision and robustness of ToF methods is limited by relying on photon time-tagging or modulation after photo-conversion. Successful optical modulation approaches have been restricted fiber-coupled modulation with large coupling losses or interferometric modulation with sub-cm range, and the precision gap between interferometric methods and ToF methods is more than three orders of magnitudes. In this work, we close this gap and propose a computational imaging method for all-optical free-space correlation before photo-conversion that achieves micron-scale depth resolution with robustness to surface reflectance and ambient light with conventional silicon intensity sensors. To this end, we solve two technical challenges: modulating at GHz rates and computational phase unwrapping. We propose an imaging approach with resonant polarization modulators and devise a novel optical dual-pass frequency-doubling which achieves high modulation contrast at more than 10GHz. At the same time, centimeter-wave modulation together with a small modulation bandwidth render existing phase unwrapping methods ineffective. We tackle this problem with a neural phase unwrapping method that exploits that adjacent wraps are often highly correlated. We validate the proposed method in simulation and experimentally, where it achieves micron-scale depth precision. We demonstrate precise depth sensing independently of surface texture and ambient light and compare against existing analog demodulation methods, which we outperform across all tested scenarios.

==> setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

%
% Old writeup from Noah
%
%We have a constant intensity CW laser at 532 nm fiber coupled into a free space setup, with polarizing optics to linearly polarize the light, beamsplitter and half wave plate, as well as a telescope to reduce the beam diameter to half a mm. That light passes through an aligned polarizing beamsplitter through a half wave plate at 22.5 degrees and a quarter waveplate at 45 degrees to elliptically polarize the light before it enters the EOM and returns from a mirror, modulating the light and adding a phase shift and acts as a retarder, passing through the QWP and HWP, flipping the polarization state from horizontal to vertical so it passes to the side of the PBS 1. It passes through another HWP, PBS 1, and QWP and then enters the scene, reflecting off the object back through the QWP and out through the right side of the PBS 2.It passes through two lenses that focus the diffuse light into another HWP and PBS, through another HWP and QWP to flip the polarization to elliptical before entering and returning from the second EOM. The light returns through the third PBS out through a lens onto an Avalanche photodetector (APD).
%
%The APD picks up the weak beat note signal from the mixing of the two EOM GHz signals, which is a DC signal varying in intensity relative to scene object position for homodyne detection with the EOMS have the same frequency, 7.15 GHz, or a sinusoidal beat note oscillating at the frequency difference between the two EOMs, in this case 1-10 kHz difference, which varies in phase relative to the clock signal. The homodyne signal is recovered by sweeping the phase with the RF driver to reconstruct the signal, smoothed with a low pass filter and RC filter, which can be fitted with a sinusoid and the phase, amplitude and bias recovered. We can also use the 4 phase method mentioned in the image formation section to recover phase and amplitude, or use an FFT to recover the phase and amplitude. For the heterodyne detection, the beat note and square wave at the same frequency from a function generator are put into a scope and triggered off the square wave, so the phase change from the object displacement is apparent and recovered from the clock signal, using an FFT to recover the phase.
%
%We also incorporate interferometry into our setup with a Michelson Interferometer used at the second PBS. A reference mirror and QWP are placed to the left of the PBS, on top of a piezoelectric stage that displaces on the order of nm's, allowing interference at the optical carrier's wavelength. The reference mirror path is varied allowing the beam from the scene $d_s$ to interfere with the reference beam $d_r$, oscillating through constructive and destructive interference. We can use the bias from the amplitude modulated setup for each mirror position to reconstruct the interference pattern and recover its phase for micron level spacial resolution. (Include figures, equations, and citations)
%
%\begin{enumerate}
  %\item Correlation.
  %\item .
  %\item .
%\end{enumerate}
